A Dynamic Improvement Framework for Vehicular Task Offloading

In this paper, the task offloading from vehicles with random velocities is optimized via a novel dynamic improvement framework. Particularly, in a vehicular network with multiple vehicles and base stations (BSs), computing tasks of vehicles are offloaded via BSs to an edge server. Due to the random velocities, the exact trajectories of vehicles cannot be predicted in advance. Hence, instead of deterministic optimization, the cell association, uplink time and throughput allocation of multiple vehicles in a period of task offloading are formulated as a finite-horizon Markov decision process. In the proposed solution framework, we first obtain a reference scheduling scheme of cell association, uplink time and throughput allocation via deterministic optimization at the very beginning. The reference scheduling scheme is then used to approximate the value functions of the Bellman's equations, and the actual scheduling action is determined in each time slot according to the current system state and approximate value functions. Thus, the intensive computation for value iteration in the conventional solution is eliminated. Moreover, a non-trivial average cost upper bound is provided for the proposed solution framework. In the simulation, the random trajectories of vehicles are generated from a high-fidelity traffic simulator. It is shown that the performance gain of the proposed scheduling framework over the baselines is significant.

==> backup/cost.tex <==
% \begin{multline}
% 	\mathsf{C}_{n,t}( \mathsf{S}_{t}, \Omega_t^H ) = \mathds{1}( 0 < d_{n,t} ) + \sum_{k =0}^{T - t}\mathds{1}\left( \sum_{\kappa = t}^{t+k} R_{n, \kappa}^{(t)} < d_{n,t} \right) + \omega_2 \max \left\{d_{n,t} - \sum_{k =0}^{T - t} {r_{n,t + k}^{(t)}}, 0\right\} \\
% 	+ \omega_1  \sum_{k =0}^{T - t} \txTime_{n,t+k} \varPhi_{n, t+k|t} 2^{\frac{r_{n,t+k}^{(t)}}{\txTime_{n,t+k} \slotLen \bandwidth}} \mathds{1}\left( \sum_{\kappa = t}^{t+k} R_{n, \kappa}^{(t)} < d_{n,t} \right) \\
% 	+ \omega_1  \sum_{k =0}^{T - t} \txTime_{n,t+k} \varPhi_{n, t+k|t} 2^{\frac{ d_{n,t} - \sum_{\kappa = t}^{t+k} R_{n, \kappa}^{(t)} }{\txTime_{n,t+k} \slotLen \bandwidth}} \mathds{1}\left( \sum_{\kappa = t}^{t+k-1} R_{n, \kappa}^{(t)} < d_{n,t} \le \sum_{\kappa = t}^{t+k} R_{n, \kappa}^{(t)} \right).
% \end{multline}

==> backup/cost_function.tex <==
\begin{figure*}[!t]
    \normalsize
    \begin{equation}
        \label{cost: case function 1}
 f_{n, t}^1(d_{n,t}, \Omega_t^H) = \begin{cases}
            0,                                                                                            & d_{n,t} \le 0,                                                                                 \\
            1 ,                                                                                           & 0 < d_{n,t} \le r_{n,t}^{(0)},                                                                 \\
            2 ,                                                                                           & r_{n,t}^{(0)} < d_{n,t} \le r_{n,t}^{(0)} + r_{n,t+1}^{(0)},                                    \\
            \ldots,                                                                                       & \ldots,                                                                                                                     \\
            \kappa+1,                                                                                     & \sum_{k = 0}^{\kappa} r_{n,t+k}^{(0)} < d_{n,t} \le \sum_{k = 0}^{\kappa+1} r_{n,t+k}^{(0)}, \\
            \ldots,                                                                                       & \ldots,                                                                                                                     \\
 T - t + \omega_2\left(d_{n,t} - \sum_{k = 0}^{T - t} {r_{n,t + k}^{(0)} }\right),               & \sum_{k = 0}^{T - t} {r_{n,t + k}^{(0)}  } < d_{n,t} \le d_{n,t}^{(0)}, \\
 T - t + \omega_2\left(d_{n,t}^{(0)} - \sum_{k =0}^{T - t} {r_{n,t + k}^{(0)}}\right), & d_{n,t}^{(0)} < d_{n, t}, 0 < \sum_{k =0}^{T - t} {r_{n,t + k}^{(0)}}, \\
 T - t + \omega_2\left(d_{n,t} - \sum_{k = 0}^{T - t} {r_{n,t + k}^{(0)}}\right), & d_{n,t}^{(0)} < d_{n, t}, 0 = \sum_{k =0}^{T - t} {r_{n,t + k}^{(0)}}, \\
        \end{cases}
    \end{equation}

    \begin{equation}
        \label{cost: case function 2}
 f_{n, t}^2(d_{n,t}, \boldsymbol{l}_{n,t} , \Omega^H) = \begin{cases}
            0,                                                                                              & d_{n,t} \le 0,                                                                                \\
 \txTime_{n,t}^{(0)} \varPhi_{n, t|t} 2^{\frac{d_{n, t}}{\txTime_{n,t}^{(0)}\slotLen \bandwidth}},                                 &  0 < d_{n,t} \le r_{n,t}^{(0)},                                                                \\
            \begin{aligned}
                & \txTime_{n,t}^{(0)} \varPhi_{n, t|t} 2^{\frac{r_{n,t}^{(0)}}{\txTime_{n,t}^{(0)}\slotLen \bandwidth}}                    \\
                & + \txTime_{n,t+1}^{(0)} \varPhi_{n, t+1|t} 2^{\frac{d_{n, t} - r_{n,t}^{(0)}}{\txTime_{n,t+1}^{(0)}\slotLen \bandwidth}}
            \end{aligned}
 ,                                                                                               & r_{n,t}^{(0)} < d_{n,t} \le r_{n,t}^{(0)} + r_{n,t+1}^{(0)},                                  \\
            \ldots,                                                                                         & \ldots,                                                                                                                    \\
            \begin{aligned}
                & \sum_{k = 0}^{\kappa }\txTime_{n,t+k}^{(0)} \varPhi_{n, t+k|t} 2^{\frac{r_{n,t+k}^{(0)}}{\txTime_{n,t+k}^{(0)} \slotLen \bandwidth}}                                   \\
                & + \txTime_{n,t+\kappa+1}^{(0)} \varPhi_{n, t+\kappa+1|t} 2^{\frac{d_{n, t} - \sum_{k = 0}^{\kappa} r_{n,t+k}^{(0)}}{ \txTime_{n,t+\kappa+1}^{(0)} \slotLen \bandwidth }}
            \end{aligned},
                                                                                                            & \sum_{k = 0}^{\kappa} r_{n,t+k}^{(0)} < d_{n,t} \le \sum_{k = 0}^{\kappa+1} r_{n,t+k}^{(0)}, \\
            \ldots,                                                                                         & \ldots,                                                                                                                    \\
            \sum_{k = 0}^{T-t}\txTime_{n,t+k}^{(0)} \varPhi_{n, t+k|t} 2^{\frac{r_{n,t+k}^{(0)}}{\txTime_{n,t+k}^{(0)}\slotLen \bandwidth}},       & \sum_{k = 0}^{T - t} {r_{n,t + k}^{(0)}} < d_{n,t} \le d_{n,t}^{(0)}, \\
            \sum_{k = 0}^{T-t}\txTime_{n,t+k}^{(0)} \varPhi_{n, t+k|t} 2^{\frac{r_{n,t+k}^{(t)}}{\txTime_{n,t+k}^{(0)}\slotLen \bandwidth}}, & d_{n,t}^{(0)} < d_{n,t}, 0 < \sum_{k =1}^{T - t} {r_{n,t + k}^{(0)}}, \\
            \sum_{k = 0}^{T-t}\txTime_{n,t+k}^{(0)} \varPhi_{n, t+k|t} 2^{\frac{r_{n,t+k}^{(0)}}{\txTime_{n,t+k}^{(0)}\slotLen \bandwidth}},       & d_{n,t}^{(0)} < d_{n,t}, 0 = \sum_{k =1}^{T - t} {r_{n,t + k}^{(0)}}. \\
        \end{cases}
    \end{equation}
    \hrulefill{}
\end{figure*}


\begin{table*}[!b]
    \centering
    \begin{tabular}{c|c|l}
    \hline
    $f_{n, t+1}^1(d_{n,t+1}, \Omega_t^H)$ & $f_{n, t + 1}^2(d_{n,t+1}, \boldsymbol{l}_{n,t+1} , \Omega_t^H)$ & Condition \\ \hline
    $0$      &$0$     & $d_{n,t+1} \le 0$           \\ \hline
    $k+1$     &        $\begin{aligned}
        & \sum_{\kappa= 1}^{k }\txTime_{n,t+\kappa}^{(0)} \varPhi_{n, t+\kappa|t+1} 2^{\frac{r_{n,t+\kappa}^{s}}{\txTime_{n,t+\kappa}^{(0)} \slotLen \bandwidth}}                                   \\
        & + \txTime_{n,t+k+1}^{(0)} \varPhi_{n, t+k+1|t+1} 2^{\frac{d_{n, t} - \sum_{\kappa= 0}^{k} r_{n,t+k}^{s}}{ \txTime_{n,t+k+1}^{(0)} \slotLen \bandwidth }}
        \end{aligned}$     &  $ \sum_{\kappa= 1}^{k} r_{n,t+k}^{s} < d_{n,t+1} \le \sum_{\kappa= 1}^{k+1} r_{n,t+k}^{s}$         \\ \hline
    $T - t + \omega_2\left(d_{n,t+1} - \sum_{\kappa= 1}^{T - t} {r_{n,t + \kappa}^{s} }\right)$  & $ \sum_{\kappa= 1}^{T-t}\txTime_{n,t+\kappa}^{(0)} \varPhi_{n, t+\kappa|t+1} 2^{\frac{r_{n,t+k}^{s}}{\txTime_{n,t+\kappa}^{(0)}\slotLen \bandwidth}}$    &  $\sum_{\kappa= 1}^{T - t} { r_{n,t+\kappa}^{s} } < d_{n,t+1}$    \\ \hline
    \end{tabular}
    \label{table: case function}
    \caption{Case functions of $f_{n, t+1}^1(d_{n,t+1}, \Omega_t^H)$ and $f_{n, t + 1}^2(d_{n,t+1}, \boldsymbol{l}_{n,t+1} , \Omega_t^H)$.}
\end{table*}


==> backup/lemma.tex <==
\begin{Lemma}
	\label{lemma: sequential improvement}
	Denote $\Omega_{t}^H$ as the base policy derived from equations \eqref{problem: reference_optimization} at the $t-1$-th slot, and $\tilde{\Omega}_{t}$ as the policy derived from \eqref{problem: rollout_policy} at the $t$-th slot. Assume the optimized policy is stationary, then \begin{equation}
		\label{eq: sequential improvement}
		\mathsf{C}_t( \mathsf{S}_t, \tilde{\Omega}_t ) \le \mathsf{C}_t( \mathsf{S}_t, \Omega_{t}^H ), \forall t.
	\end{equation}
\end{Lemma}
\begin{proof}
	Similar to the proof in \cite{bertsekas2019reinforcement}.
	Apparently inequality \eqref{eq: sequential improvement} is satisfied when $t = T$, since
	\begin{equation}
		\min_{\mathsf{A}_T} \mathsf{c}_T(\mathsf{S}_T, \mathsf{A}_T) \le  \mathsf{c}_T\left(\mathsf{S}_T, \Omega_{t}^H(\mathsf{S}_T)\right)
	\end{equation}
	Assume inequality \eqref{eq: sequential improvement} satisfied, that is $\mathsf{C}_{t+1}( \mathsf{S}_{t+1}, \tilde{\Omega}_{t+1} ) \le \mathsf{C}_{t+1}( \mathsf{S}_{t+1}, \Omega_{t+1}^H )$. Then we have
	\begin{equation}
		\begin{aligned}
			\mathsf{C}_t( \mathsf{S}_t, \tilde{\Omega}_{t} ) &= \mathbb{E}_{\mathsf{S}_{t+1}} \left[ \mathsf{c}_t(\mathsf{S}_t, \tilde{\Omega}_{t}(\mathsf{S}_t)) + \mathsf{C}_{t+1}( \mathsf{S}_{t+1}, \tilde{\Omega}_{t+1} ) \right] \\
			&\le  \mathbb{E}_{\mathsf{S}_{t+1}} \left[ \mathsf{c}_t(\mathsf{S}_t, \tilde{\Omega}_{t}(\mathsf{S}_t)) + \mathsf{C}_{t+1}( \mathsf{S}_{t+1}, \Omega_{t+1}^H ) \right] \\
			&=  \mathbb{E}_{\mathsf{S}_{t+1}} \left[ \mathsf{c}_t(\mathsf{S}_t, \tilde{\Omega}_{t}(\mathsf{S}_t)) +  \mathcal{H}_{t}^\star(\mathsf{S}_{t}, \mathsf{A}_{t}) + \mathsf{C}_{t+1}( \mathsf{S}_{t+1}, \Omega_{t+1}^H ) -  \mathcal{H}_{t}^\star(\mathsf{S}_{t}, \mathsf{A}_{t}) \right]\\
			&=    \min_{\mathsf{A}_t} \left\{ \mathsf{c}_t(\mathsf{S}_t, \mathsf{A}_t) +  \mathcal{H}_{t}^\star(\mathsf{S}_{t}, \mathsf{A}_{t})  \right\} -  \mathcal{H}_{t}^\star(\mathsf{S}_{t}, \mathsf{A}_{t}) + \mathbb{E}_{\mathsf{S}_{t+1}} \left[\mathsf{C}_{t+1}( \mathsf{S}_{t+1}, \Omega_{t+1}^H )  \right]\\	
			&\le \mathbb{E}_{\mathsf{S}_{t+1}} \left[ \mathsf{c}_t(\mathsf{S}_t, \mathsf{A}_t) + \mathsf{C}_{t+1}( \mathsf{S}_{t+1}, \Omega_{t+1}^H ) \right] \\
			&= \mathsf{C}_t( \mathsf{S}_t, \Omega_{t}^H ),
		\end{aligned}
	\end{equation}
	where the second inequality results from $\min_{\mathsf{A}_t}  \left\{ \mathsf{c}_t(\mathsf{S}_t, \mathsf{A}_t) + \mathcal{H}_t^\star(\mathsf{S}_{t}, \mathsf{A}_t) \right\} \le  \mathsf{c}_t(\mathsf{S}_t, \mathsf{A}_t) + \mathcal{H}_t^\star(\mathsf{S}_{t}, \mathsf{A}_t)$
\end{proof}

From the \lemmaref{lemma: sequential improvement}, we can say the policy derived from \eqref{problem: rollout_policy} is better than the policy derived from \eqref{problem: reference_optimization} in each $t$-th time slot. 

==> backup/preallocation.tex <==

\subsection{Offline Pre-Allocation}
The phase of offline pre-allocation is to provide a baseline of scheduling actions for all the vehicles in all the time slots, which can be exploit to approximate the value function of the Bellman's equations in \eqref{equation: Bellman}. In this part, we choose the average trajectories for all the vehicles as follows:
\begin{equation}
    \boldsymbol{l}_{n,t}^{(0)} = \mathbb{E}\left[ \boldsymbol{l}_{n,t} | \boldsymbol{l}_{n,0}\right], \forall n, t.
\end{equation}
Then the BS association and time allocation of the pre-allocation is given by
\begin{equation}
	e_{n, m, t} = \mathds{1}\left(m = \argmax_{m \in \mathcal{M}} \mathbb{E}_h\left[ \vert hg_{n,m,t} \vert^2 \right]\right), 
\end{equation}
and
\begin{equation}
	\txTime_{n,t} = \frac{1}{ \left[\mathbf{1}^T \boldsymbol{E}_t \right]_m}.
\end{equation}

Moreover, assuming all the vehicles are moving along the average trajectories, the expectation on the random trajectories in \eqref{equation: Bellman} can be omitted. Hence, adopting the above BS association and time allocation, the optimization of throughput allocation in (xx) can be simplified as 
...

\begin{equation}
	\Problem
	\begin{aligned}
		\min_{ \substack{\left\{ r_{n,T_n^a}, \ldots, r_{n,t} \right\} \\ \{ t_1^d, \ldots, t_N^d \}} } \quad & {\Delta T}_n  + \omega_1 \sum_{T_n^a \le t \le t_n^d} P_{n, t} \txTime_{n, t} \\
		&+ \omega_2 \left(D_n^a - \sum_{T_n^a \le t \le t_n^d} r_{n,t}  \right) \\
		\text{s.t.}  \quad
		 & \Delta T_n = t_n^d  - T_n^a + (T - t_n^d)\mathds{1}(d_{n,T} > 0) , \\
		 & t_n^d \le T, \\
		 & -r_{n,t} \le 0, \forall t, \\
		 & P_{n,t} \le P_{\max},  \\
		 & P_{n,t} =  2^{\frac{r_{n,t}}{\txTime_{n,t} \slotLen \bandwidth }}\Phi_{n,t}, \forall t.
	\end{aligned}
\end{equation}
The above problem can be infeasible due to the power constraint $P_{n,t} \le P_{\max}$.
Therefore, the time slots we interested in the optimization is only $\mathcal{T}_n \triangleq \left\{t \middle | \Phi_{n,t} > P_{\max} \right\}$.
Based on the different $t_n^d$, the problem can be solved accordingly.
\subsubsection{Case 1, $ t_n^d \le T$ and $d_{n,T} = 0$}
Given a fixed ${\Delta T}_n$, the transmission time cost is determined, and by default, the task is guaranteed to be completed.
Therefore, the target is to solve an energy minimization problem.
\begin{equation}
	\Problem
	\begin{aligned}
		\min_{ \left\{ r_{n,t} \middle | t \in \mathcal{T}_n, t \le t_n^d \right\} } \quad & \omega_1 \sum_{t \in \mathcal{T}_n, t \le t_n^d} 2^{\frac{r_{n,t}}{\txTime_{n,t} \slotLen \bandwidth }} \Phi_{n,t} \txTime_{n, t} \\
		\text{s.t.}  \quad
		& -r_{n,t} \le 0, \forall t, \\
		& r_{n,t} \le \txTime_{n,t} \slotLen \bandwidth \log_2 \frac{P_{\max}}{\Phi_{n,t}}, \forall t. \\
		& D_n^a = \sum_{t \in \mathcal{T}_n, t \le t_n^d} r_{n,t}. 
	\end{aligned}
\end{equation}
% The Lagrange function of the above problem is given by
% \begin{multline}
% 	L(\boldsymbol{R}_n, \boldsymbol{\lambda}_n, \mu_n) = \omega_1 \sum_{t \in \mathcal{T}_n, t \le t_n^d} 2^{\frac{r_{n,t}}{\txTime_{n,t} \slotLen \bandwidth }} \Phi_{n,t} \txTime_{n, t} \\ - \sum_{t \in \mathcal{T}_n, t \le t_n^d}\lambda_{n,t}r_{n,t} + \mu_{n} \left( \sum_{t \in \mathcal{T}_n, t \le t_n^d}  r_{n,t} - D_n^a \right) \\  + \sum_{t \in \mathcal{T}_n, t \le t_n^d} \nu_{n,t} \left( r_{n,t} - \txTime_{n,t} \slotLen \bandwidth \log_2 \frac{P_{\max}}{\Phi_{n,t}} \right) ,
% \end{multline}
and the KKT conditions for the above problem are given by
\begin{equation}
	\begin{aligned}
		\frac{\partial L}{\partial r_{n,t}} = \omega_1' 2^{\frac{r_{n,t}}{\txTime_{n,t} \slotLen \bandwidth }} \Phi_{n,t} {\ln 2} - \lambda_{n,t} + \nu_{n,t}  + \mu_n & = 0    \\
		\lambda_{n,t} r_{n,t} = 0, \nu_{n,t} \left( r_{n,t} - \txTime_{n,t} \slotLen \bandwidth \log_2 \frac{P_{\max}}{\Phi_{n,t}} \right) &= 0  \\
		\sum_{t \in \mathcal{T}_n, t \le t_n^d} r_{n,t} - D_n^a & = 0,   \\
		\lambda_{n,t}                                                                                                                       \ge 0, \nu_{n,t} &\ge 0.  \\
	\end{aligned}
\end{equation}
where $\omega_1' = \frac{\omega_1}{\slotLen \bandwidth}$.
Therefore, the solution can be given by
\begin{equation}
	\label{eqaution: reference rate compute 1}
	\mu_n = - \omega_1' \Phi_{n,t} \ln 2 \cdot 2^{\frac{r_{n,t}}{\txTime_{n,t} \slotLen \bandwidth}}, \forall r_{n,t} \in (0, \txTime_{n,t} \slotLen \bandwidth \log_2 \frac{P_{\max}}{\Phi_{n,t}}).
\end{equation}

As for the time slot when the power is not allocated or the power is allocated at the limitation, the $\mu_n$ should satisfy corresponding constraints, that is
\begin{equation}
	\label{eqaution: reference rate compute 2}
	\mu_n \ge  - \omega_1' \Phi_{n,t} \ln 2,
\end{equation}
and 
\begin{equation}
	\mu_n \le  - \omega_1' P_{\max} \ln 2.
\end{equation}
It is evident that these two conditions cannot coexist, as $\Phi_{n,t} > P_{\max}$ for all $t \in \mathcal{T}$. 
Consequently, a water-filling-like approach can be utilized.
Let $\mathcal{T}{n}^1$ denote the set of time slots where the allocated power does not reach the power limit, and $\mathcal{T}{n}^2$ represent the set of time slots where the power is allocated at the power limit.
By expressing the transmission rate as a function of $\mu_n$, the optimal solution can be derived by first determining $\mu_n$ from
\begin{equation}
	\begin{aligned}
		D_n^a & = \sum_{t \in \mathcal{T}_{n}^1} \txTime_{n,t} \slotLen \bandwidth \log_2 \frac{-\mu_n }{\omega_1' \Phi_{n,t} \ln 2 } + \sum_{t \in \mathcal{T}_{n}^2} \txTime_{n,t} \slotLen \bandwidth \log_2 \frac{ P_{\max} }{ \Phi_{n,t} }. \\
	\end{aligned}
\end{equation}
% That is
% \begin{equation}
% 	\mu_n = -2^{\frac{D_n^a +  \sum_{t} \txTime_{n,t} \slotLen \bandwidth \log_2 \omega_1' \Phi_{n,t} \ln 2}{ \sum_{t} \txTime_{n,t} \slotLen \bandwidth}}.
% \end{equation}
Once the feasible $\mu_n$ is found, the optimal $ r_{n,T_n^a}, \ldots, r_{n,t_n^d}$ can be derived accordingly with \eqref{eqaution: reference rate compute 1} and \eqref{eqaution: reference rate compute 2}.
\subsubsection{Case 2, $t_n^d = T$, and $0 < d_{n,T}$}
In this case, the optimization problem can be transformed into
\begin{equation}
	\Problem
	\begin{aligned}
		\min_{  r_{n,T_n^a}, \ldots, r_{n,T} } \quad & \omega_1 \sum_{t \in \mathcal{T}_n} 2^{\frac{r_{n,t}}{\txTime_{n,t} \slotLen \bandwidth}} \Phi_{n,t} \txTime_{n, t}  \\ 
		 & +  \omega_2 \left(D_n^a - \sum_{t \in \mathcal{T}_n} r_{n,t} \right) \\
		\text{s.t.}  \quad
		 & -r_{n,t} \le 0, \forall t,                                                                                                                                          \\
		 & \sum_{t \in \mathcal{T}_n} r_{n,t} < D_n^a,  \\
		 & r_{n,t} \le \txTime_{n,t} \slotLen \bandwidth \log_2 \frac{P_{\max}}{\Phi_{n,t}}, \forall t. \\
	\end{aligned}
\end{equation}
where the constant $T - t_n^d$ at the target function is omitted without changing the optimal solution.
% The Lagrange function of the above problem is given by
% \begin{multline}
% 	L(\boldsymbol{R}_n, \boldsymbol{\lambda}_n) = \omega_1 \sum_{t \in \mathcal{T}_n} 2^{\frac{r_{n,t}}{\txTime_{n,t} \slotLen \bandwidth}} \Phi_{n,t} \txTime_{n, t} - \sum_{t \in \mathcal{T}_n}\lambda_{n,t}r_{n,t} \\ + \sum_{t \in \mathcal{T}_n} \nu_{n,t} \left( r_{n,t} - \txTime_{n,t} \slotLen \bandwidth \log_2 \frac{P_{\max}}{\Phi_{n,t}} \right) \\ + \left(\mu_{n} - \omega_2\right) \left( \sum_{t \in \mathcal{T}_n} r_{n,t} - D_n^a \right),
% \end{multline}
The KKT conditions for the above problem are given by
\begin{equation}
	\begin{aligned}
		\frac{\partial L}{\partial r_{n,t}} = \omega_1' 2^{\frac{r_{n,t}}{\txTime_{n,t}\slotLen \bandwidth}} \Phi_{n,t} \ln 2 - \lambda_{n,t} + \nu_{n,t} + \left(\mu_{n} - \omega_2\right) & = 0  \\
		\lambda_{n,t} r_{n,t} = 0, \nu_{n,t} \left( r_{n,t} - \txTime_{n,t} \slotLen \bandwidth \log_2 \frac{P_{\max}}{\Phi_{n,t}} \right) &= 0 \\
		\mu_n \left(\sum_{t \in \mathcal{T}_n} r_{n,t}  - D_n^a\right) & = 0, \\
		\lambda_{n,t} \ge 0, \nu \ge 0, \mu_n & = 0. \\
	\end{aligned}
\end{equation}
Therefore, the solution can be given by
\begin{equation}
	r_{n,t} = \begin{cases}
		0,  & \omega_1' \Phi_{n,t} \ln 2 \ge \omega_2, \\
		\txTime_{n,t} \slotLen \bandwidth \log_2 \frac{P_{\max}}{\Phi_{n,t}}, & \omega_1' P_{\max} \ln 2 \le \omega_2, \\
		\txTime_{n,t} \slotLen \bandwidth \log_2 \frac{\omega_2}{\omega_1' \Phi_{n,t} \ln 2}, & \text{otherwise}.
	\end{cases}
\end{equation}


==> backup/solution.tex <==
\begin{comment}


    This approach leverages knowledge of the current system state and predictions of future trajectories. 
    Rather than solving the Bellman equation from the $T$-th time slot backward for all possible system states, the proposed method solves the problem in the following four steps:
    1) First, we derived a pre-allocation based on a prediction of future trajectory;
    2) Using the location transmission matrix, the expected analytical performance of the pre-allocation is then calculated; 
    3) Next, optimization is performed in each $t$-th time slot based on the current system state and the pre-allocation;
    4) Finally, since the pre-allocation is derived from predicted future trajectories, its feasibility is further verified against the actual system state.
    
    With the introducing of auxiliary parameter $\{ t_1^d, \ldots, t_N^d \}$, the optimization problem is formulated as
    \begin{equation}
     \Problem
      \begin{aligned}
     \min_{ \substack{\left\{ \mathsf{A}_1, \ldots, \mathsf{A}_T \right\} \\ \{ t_1^d, \ldots, t_N^d \}} } \quad & \mathbb{E} \left[ \sum_{n \in \mathcal{N}} \left( {\Delta T}_n + \omega_1 \sum_{t = 0}^{T-1} P_{n, t} \txTime_{n, t} + \omega_2 d_{n,T}\right) \middle | \mathsf{S}_0 \right] \\
     \text{s.t.} \quad
        & \textit{C1}, \textit{C2}, \textit{C3}, \textit{C4}                     \\
        & \Delta T_n = t_n^d - T_n^a + (T - t_n^d)\mathds{1}(d_{n,T} > 0), \forall n,  \\
        & t_n^d \le T, \forall n,                             \\
        & D_n^a - d_{n,T} = \sum_{T_n^a \le t < t_n^d} r_{n,t}, \forall n,        \\
        & P_{n,t} \le P_{\max},
      \end{aligned}
    \end{equation}
    where in the target function, the first part $ \Delta T_n $ represents the transmission time cost for task $n$, the second part $\sum_{t=0}^{T-1} P_{n,t}\txTime_{n,t}$ is energy consumption of the vehicle, and the last part $d_{n, T}$ represents a penalty of an uncompleted transmission.
    
    
    
    Denote pre-allocations as $\Omega^H = \left(\Omega_0^H, \Omega_1^H, \ldots, \Omega_T^H \right)$.
    The initial pre-allocation $\Omega_0^H: t \mapsto \mathsf{A}_{t}$ is derived by solving the optimization problem \ref{problem: finite MDP} with the trajectory predicted as the average trajectory.
    \begin{equation}
    \label{problem: reference_optimization}
    \Omega^H_0 = \argmin_{ \mathsf{A}_{0}, \mathsf{A}_{1}, \ldots, \mathsf{A}_{T} } \quad \sum_{ t = 0 }^ {T} \mathsf{c}_{t} ( \boldsymbol{d}_{t} , \mathbb{E}\left[ \boldsymbol{L}_{t} | \boldsymbol{L}_{0} \right], \mathsf{A}_{t}).
    \end{equation}
    
    On top of the initial pre-allocation, the pre-allocation $\Omega_\zeta^H: \mathsf{S}_{\zeta-1}, t \mapsto \mathsf{A}_{t}$ is further modified based on the given system state $\mathsf{S}_{\zeta-1}$.
    For each $n$-th vehicle, the initial policy $\Omega_0^H$ defines the transmitted transmission rate $r_{n,t}^{(0)}$, and allocated transmission time $\txTime_{n,t}^{(0)}$ in each $t$-th slot.
    Therefore, the task transmission slot numbers and the information bits left to be transmitted at each $t$-th slot can determined as $t_n^{(0)}$, and $d_{n,t}^{(0)} = d_{n,0} - \sum_{t = 0}^{t-1} r_{n,t}^{(0)}$.
    
    After optimizing the above problem \eqref{problem: reference_optimization}, the optimized scheduling in $t$-th slot is given by solving the Bellman equation \eqref{equation: Bellman}, where the value function at the next time slot $t+1$ is approximated by total cost derived from the pre-allocation $\Omega_{t+1}^H$. 
    The optimal solution $\tilde{\Omega}(\mathsf{S}_t)$ is given by
    \begin{equation}
    \label{problem: rollout_policy}
    \argmin_{\mathsf{A}_{t}} \left\{ \mathsf{c}_t(\mathsf{S}_t, \mathsf{A}_t) + \sum_{\mathsf{S}_{t+1}} \mathbb{P}\left[ \mathsf{S}_{t+1} \middle | \mathsf{S}_t \right] \mathsf{C}_{t+1}( \mathsf{S}_{t+1}, \Omega^H_{t+1} ) \right\}.
    \end{equation}
    Therefore, by computing equation \eqref{problem: rollout_policy} in each $t$-th time slot, the approximated policy $\tilde{\Omega}$ can be obtained.
    
    Moreover, due to different optimized solutions chosen in the last slot, the actual remaining information bits $d_{n,t}$ might be different from the one computed with pre-allocation, affecting the approximation performance of the pre-allocation.
    Therefore, the pre-allocation is further updated based on the following equation
    \begin{equation}
     r_{n,t}^{(\zeta)} = \begin{cases}
     \frac{ d_{n,\zeta} }{ \sum_{\zeta \le t} r_{n,t}^{(0)} } r_{n,t}^{(0)}, & d_{n,\zeta} > d_{n,\zeta}^{(0)}, 0 < \sum_{\zeta \le t} r_{n,t}^{(0)} \\
     r_{n,t}^{(0)},& \text{otherwise},
    \end{cases}, \forall \zeta \le t.
    \end{equation}
    
    
    \end{comment}
